Using Neural Networks to Compute Approximate and Guaranteed Feasible Hamilton-Jacobi-Bellman PDE Solutions

To sidestep the curse of dimensionality when computing solutions to Hamilton-Jacobi-Bellman partial differential equations (HJB PDE), we propose an algorithm that leverages a neural network to approximate the value function. We show that our final approximation of the value function generates near optimal controls which are guaranteed to successfully drive the system to a target state. Our framework is not dependent on state space discretization, leading to a significant reduction in computation time and space complexity in comparison with dynamic programming-based approaches. Using this grid-free approach also enables us to plan over longer time horizons with relatively little additional computation overhead. Unlike many previous neural network HJB PDE approximating formulations, our approximation is strictly conservative and hence any trajectories we generate will be strictly feasible. For demonstration, we specialize our new general framework to the Dubins car model and discuss how the framework can be applied to other models with higher-dimensional state spaces.

==> Bibliography.tex <==
% !TEX root = NNET_HSCC.tex

\begin{thebibliography}{1}

\bibitem{theory1} P. Varaiya, “On the existence of solutions to a differential game,” \textit{SIAM
Journal on Control}, vol. 5, no. 1, pp. 153–162, 1967.
\bibitem{theory2} L. C. Evans and P. E. Souganidis, “Differential games and representation
formulas for solutions of Hamilton-Jacobi-Isaacs equations,”
\textit{Indiana Univ. Math. J.}, vol. 33, no. 5, pp. 773–797, 1984.
\bibitem{theory3} E. Barron, "Differential Games with Maximum Cost," \textit{Nonlinear
analysis: Theory, methods \& applications}, pp. 971–989, 1990.
\bibitem{theory4} C. J. Tomlin, J. Lygeros, and S. S. Sastry, “A game theoretic approach
to controller design for hybrid systems,” \textit{Proceedings of the IEEE},
vol. 88, no. 7, pp. 949 –970, July 2000.
\bibitem{theory5} I. Mitchell, A. Bayen, and C. Tomlin, “A time-dependent HamiltonJacobi
formulation of reachable sets for continuous dynamic games,”
\textit{IEEE Transactions on Automatic Control}, vol. 50, no. 7, pp. 947–957,
July 2005.
\bibitem{theory6} O. Bokanowski, N. Forcadel, and H. Zidani, “Reachability and minimal
times for state constrained nonlinear problems without any controllability
assumption,” \textit{SIAM Journal on Control and Optimization},
pp. 1–24, 2010.
\bibitem{theory7} J. F. Fisac, M. Chen, C. J. Tomlin, and S. S. Shankar, “Reach-avoid
problems with time-varying dynamics, targets and constraints,” in
\textit{18th International Conference on Hybrid Systems: Computation and
Controls}, 2015.

\bibitem{refueling} J. Ding, J. Sprinkle, S. S. Sastry, and C. J. Tomlin, “Reachability
calculations for automated aerial refueling,” in \textit{IEEE Conference on
Decision and Control}, Cancun, Mexico, 2008.
\bibitem{platooning} M. Chen, Q. Hu, C. Mackin, J. Fisac, and C. J. Tomlin, “Safe
platooning of unmanned aerial vehicles via reachability,” in \textit{IEEE
Conference on Decision and Control}, 2015.
\bibitem{projections} I. M. Mitchell and C. J. Tomlin, “Overapproximating reachable sets by
hamilton-jacobi projections,” \textit{Journal of Scientific Computing}, vol. 19,
no. 1-3, pp. 323–346, 2003.
\bibitem{dp} J. S. McGrew, J. P. How, L. Bush, B. Williams, and N. Roy, “Air
combat strategy using approximate dynamic programming,” \textit{AIAA
Guidance, Navigation, and Control Conference}, Aug 2008.
\bibitem{disturbances} M. Chen*, S. Herbert*, and C. J. Tomlin, “Fast reachable set approximations
via state decoupling disturbances,” in \textit{55th IEEE Conference
on Decision and Control}, 2016.

\bibitem{restrictive1} A. Majumdar and R. Tedrake, \textit{Algorithmic Foundations of Robotics X:
Proceedings of the Tenth Workshop on the Algorithmic Foundations
of Robotics}. Springer Berlin Heidelberg, 2013, ch. Robust Online
Motion Planning with Regions of Finite Time Invariance, pp. 543–
558.
\bibitem{restrictive2} T. Dreossi, T. Dang, and C. Piazza, “Parallelotope bundles for polynomial
reachability,” in \textit{19th International Conference on Hybrid
Systems: Computation and Controls}, 2016.
\bibitem{restrictive3} J. Darbon and S. Osher, “Algorithms for overcoming the curse of
dimensionality for certain hamilton-jacobi equations arising in control
theory and elsewhere,” \textit{arXiv preprint arXiv}:1605.01799, 2016.

%\bibitem{IEEEhowto:kopka}
%H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  %0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

\bibitem{nnet_becerikli} Y. Beceriklia, A. Konarb, T. Samad. "Intelligent optimal control with dynamic neural networks". \textit{Neural Networks 16} (2003) 251–259.

\bibitem{nnet_lau}
K. Lau, R. Lopez and E. Onate. "Neural Networks for Optimal Control of Aircraft Landing Systems". \textit{Proceedings of the World Congress on Engineering}, 2007.

\bibitem{nnet_stanford}
R. Allen, A. Clark, J. Starek, and M. Pavone. "A Machine Learning Approach for Real-Time Reachability Analysis". \textit{International Conference on Intelligent Robots and Systems}, 2014.

\bibitem{nnet_lygeros}
B. ~Djeridane and J. ~Lygeros, \emph{Neural approximation of PDE solutions: An application to
reachability computations}. \hskip 1em plus 0.5 em minus 0.4em\relax 
IEEE Conference on Decision and Control 2006, pages 3034-3039. IEEE, 2006.

\bibitem{nnet_niarchos}
K. N. Niarchos and J. Lygeros, \emph{A Neural Approximation to Continuous Time Reachability Computations}. \hskip 1em plus 0.5 em minus 0.4em\relax 
IEEE Conference on Decision and Control 2006, pages 6313-6318. IEEE, 2006.

\bibitem{accept-reject}
C.P.Robert and G. Cassela, \emph{Monte Carlo Statistical Methods},
Springer-Verlag; 2004.

\bibitem{tetra}
Timothy J. Barth, James A. Sethian. \emph{Numerical Schemes for the Hamilton–Jacobi and Level Set Equations
on Triangulated Domains}.\hskip 1em plus 0.5 em minus 0.4em\relax Journal of Computational Physics, Volume 145, Issue 1, 1 September 1998, Pages 1-40. 

\bibitem{dubins}
L. E. Dubins. \emph{On curves of minimal length with a constraint on average curvature and with prescribed
initial and terminal positions and tangents}.\hskip 1em plus 0.5 em minus 0.4em\relax American Journal of Mathematics, 79:497–516, 1957.

\bibitem{tesla}
Fortune. (2016) Feds Say Safety Is the Key to the Future of Autonomous Cars. [Online]. Available: http://fortune.com/2016/07/19/safety-feds-autonomous-cars/
\bibitem{drones1}
Jointed Planning and Development Office (JPDO), “Unmanned aircraft systems (UAS) comprehensive plan – a report on the nation’s UAS path forward,” Federal Aviation Administration, Tech. Rep., 2013.
\bibitem{drones2} Amazon.com, Inc. (2016) Amazon prime air. [Online]. Available: http://www.amazon.com/b?node=8037720011
\bibitem{drones3} BBC Technology. (2016) Google plans drone delivery
service for 2017. [Online]. Available: http://www.bbc.com/news/
technology-34704868
\bibitem{drones4} AUVSI News. (2016) Uas aid in south carolina tornado investigation.
[Online]. Available: http://www.auvsi.org/blogs/auvsi-news/2016/01/
29/tornado
\bibitem{drones5} National Aeronautics and Space Administration. (2016) Challenge is
on to design sky for all. [Online]. Available: http://www.nasa.gov/
feature/challenge-is-on-to-design-sky-for-all
\bibitem{hj_pde1} M. G. Crandall and P.-L. Lions, “Viscosity solutions of Hamilton-Jacobi
equations,” \textit{Transactions of the American Mathematical Society},
vol. 277, no. 1, pp. 1–42, 1983.
\bibitem{hj_pde2} M. G. Crandall, L. C. Evans, and P. L. Lions, “Some properties of
viscosity solutions of hamilton-jacobi equations,” \textit{Transactions of the
American Mathematical Society}, vol. 282, no. 2, p. 487, April 1984.
\bibitem{hj_ttr} I. Yang, S. Becker-Weimann, M. J. Bissell, C. J. Tomlin, "One-Shot Computation of Reachable Sets for Differential Games," \textit{HSCC '13 Proceedings of the 16th international conference on Hybrid systems: computation and control}, pages 183-192.

\bibitem{glorot} Xavier Glorot, Antoine Bordes, and Yoshua Bengio. ``Deep Sparse Rectifier
Networks''. In \textit{AISTATS}, pp. 315-323, 2011.
\bibitem{cybenko} G. Cybenko, ``Approximation by Superposition of a Sigmoidal
Function'', \textit{Math. Control Signals Systems}, vol. 2, 1989,
pp 303-314.
\end{thebibliography}


==> method_summary.tex <==
% !TEX root = NNET_HSCC.tex
\section{Summary of Method}\label{sec:method_summary}
We seek to overcome these challenges faced by dynamic programming-based
approaches by computing an approximation of $\ttr(\state)$ \textit{only in a region around} the trajectory from $\state$ to $\targetset$. For simplicity, we will assume that the target set contains a single point: $\targetset = \{\state_\targetset\}$. Afterwards, a controller can be synthesized based on the approximate TTR function $\hat\ttr(\state)$ according to \eqref{eq:opt_control}. Our method involves two phases: an NN training phase and a controller synthesis phase. 

In the NN training phase, we train an NN to understand the dynamics of the system in order to synthesize control sequences $\hat\ctrl_i(\cdot)$ such that the resulting backward-time trajectories $\hat\state_i = \traj_i^{-\dyn}(\hat T_i; \state_\targetset, 0, \hat\ctrl_i(\cdot))$ are near some state of interest $\bar\state$. Since the dynamics $\dyn$ are time-invariant, the duration of the trajectory $\hat T_i$ is an estimate of the TTR function: $\hat T_i = \hat\ttr(\hat\state_i)$. Since the trajectories satisfy the system dynamics, the TTR estimate is always conservative: $\hat\phi(\state) \ge \phi(\state)$.

At the beginning of the training process, the NN is not able to determine which control sequences $\{\hat\ctrl_i(\cdot)\}$ would result in a set $\{\hat\state_i\}$ that contains many states near $\bar\state$. Through many dynamica training iterations, eventually the states in $\{\hat\state_i\}$ become very close to $\bar\state$. Note that if any state in the set $\{\hat\state_i\}$, say $\hat\state_k$ is exactly equal to $\bar\state$, then from $\bar\state$ we can simply use \eqref{eq:backward_traj} and apply $\hat\ctrl_k(\cdot)$ to drive the system from $\bar\state$ to $\state_\targetset$: $\state_\targetset = \traj^\dyn(\hat T_i; \bar\state, 0; \hat\ctrl_k(\cdot))$. This is in general neither possible nor robust, leading to the controller synthesis phase.

In the controller synthesis phase, we start with the TTR function estimate $\hat\ttr(\state)$ on the points $\hat\state_i$, and apply the corresponding controls $\hat\ctrl_i(\cdot)$ to populate $\hat\ttr(\cdot)$ also on points along the trajectories $\traj_i^{-\dyn}(t; \state_\targetset, 0, \hat\ctrl_i(\cdot)), t \in [0, T_i]$. From this process, we obtain $\hat\ttr(\state)$ in a dynamically feasible  ``corridor'' from $\bar\state$ to $\state_\targetset$. Finally, $\hat\ttr(\state)$ can be used to synthesize a controller according to \eqref{eq:opt_control}.
